BANF: Band-limited Neural Fields for Levels of Detail Reconstruction

Largely due to their implicit nature, neural fields lack a direct mechanism for filtering, as Fourier analysis from discrete signal processing is not directly applicable to these representations. Effective filtering of neural fields is critical to enable level-of-detail processing in downstream applications, and support operations that involve sampling the field on regular grids (e.g. marching cubes). Existing methods that attempt to decompose neural fields in the frequency domain either resort to heuristics or require extensive modifications to the neural field architecture. We show that via a simple modification, one can obtain neural fields that are low-pass filtered, and in turn show how this can be exploited to obtain a frequency decomposition of the entire signal. We demonstrate the validity of our technique by investigating level-of-detail reconstruction, and showing how coarser representations can be computed effectively.

==> fig/3d-abl.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.32\textwidth, height=7em]{example-image-golden}
\hfill
\includegraphics[width=.32\textwidth, height=7em]{example-image-golden}
\hfill
\includegraphics[width=.32\textwidth, height=7em]{example-image-golden}
\hfill
\\
\end{center}
\caption{\textbf{3D Ablation}. We compare applying our decomposition method on the geometry and the color neural fields.}
\label{fig:3d-abl}
\end{figure*}

==> fig/bacon_comp.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width= \textwidth]{fig/bacon_comp_1.jpeg}
\end{center}
% 
\vspace{-1em}
\caption{
%  
%
}
\label{fig:2d_comp_1}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width= \textwidth]{fig/bacon_comp_2.jpeg}
\end{center}
% 
\vspace{-1em}
\caption{
%  
%
}
\label{fig:2d_comp_2}
\end{figure*}

==> fig/diff_inter.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width= \textwidth]{fig/diff_interpolation_1.jpg}
\end{center}
% 
\vspace{-1em}
\caption{
%  

}
\label{fig:diff_inter_1}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width= \textwidth]{fig/diff_interpolation_2.jpg}
\end{center}
% 
\vspace{-1em}
\caption{
%  
}
\label{fig:diff_inter_2}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width= \textwidth]{fig/diff_interpolation_3.jpg}
\end{center}
% 
\vspace{-1em}
\caption{
%  
}
\label{fig:diff_inter_3}
\end{figure*}

==> tab/2d.tex <==
\begin{table}[]
\centering
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{} & \multicolumn{5}{c}{PSNR~$\uparrow$ / SSIM~$\uparrow$} \\
Method & 1/8x & 1/4x & 1/2x & 1x & Average \\
\midrule
BACON & -/- & -/- & -/- & -/- & -/-  \\
PNF & -/- & -/- & -/- & -/- & -/- \\
BANF & -/- & -/- & -/- & -/- & -/- \\
\bottomrule
\end{tabular}
\caption{2D Image Results. \TODO{Generate these metrics}}
\label{tab:2d}
\end{table}

\captionof{table}{
% 
\textbf{Inverse rendering} --
Quantitative results for NeUS~\cite{wang2021neus} LOD reconstruction on the Synthetic NeRF Dataset~\cite{barron2021mipnerf}. See qualitative results in \Cref{fig:3d}. Metric is Chamfer Distance ($\times 10^{-2}) $~$\downarrow$.
%
}

==> tab/3D_color_supp_old.tex <==
\begin{table*}[!tb]
\begin{tabular}{ccc|cc}
         & iNGP-64 & BANF-64 & iNGP-128 & BANF-128 \\ \hline
Chair    &    26.27     &         &          &          \\
Drums    &    21.85     &         &          &          \\
Ficus    &    24.06     &         &          &          \\
Hotdog   &    28.33     &         &          &          \\
Lego     &         &         &          &          \\
Material &         &         &          &          \\
Mic      &         &         &          &          \\
Ship     &         &         &          &          \\ \hline
Average  &         &         &          &         
\end{tabular}
\label{fig:3d-color}
\end{table*}

==> tab/3d-abl.tex <==
\begin{table}[]
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{2}{c}{Decomposition} & \multicolumn{5}{c}{Chamfer~$\downarrow$ / PSNR~$\uparrow$} \\
 & Geom. & Color & 1/8x & 1/4x & 1/2x & 1x & Avg. \\ \midrule
\multirow{3}{*}{Blender} &  &  & -/- & -/- & -/- & -/- & -/- \\
 & \checkmark &  & -/- & -/- & -/- & -/- & -/- \\
 & \checkmark & \checkmark & -/- & -/- & -/- & -/- & -/- \\ \midrule
\multirow{3}{*}{DTU} &  &  & -/- & -/- & -/- & -/- & -/- \\
 & \checkmark &  & -/- & -/- & -/- & -/- & -/- \\
 & \checkmark & \checkmark & -/- & -/- & -/- & -/- & -/- \\ \bottomrule
\end{tabular}
\caption{3D Geometry Ablation. We compare applying our decomposition method on the geometry and the color neural fields. \TODO{Unlikely we will get this for submission, but we can do this in supplementary}}
\label{tab:3d}
\end{table}

==> tab/3d-dtu.tex <==
\begin{table*}[]
\centering
\begin{tabular}{cccccccccccccccccc}
\toprule
\multirow{2}{*}{Scale} & \multirow{2}{*}{Method} & \multicolumn{16}{c}{Chamfer~$\downarrow$ / PSNR~$\uparrow$} \\
 &  & 24 & 37 & 40 & 55 & 63 & 65 & 69 & 83 & 97 & 105 & 106 & 110 & 114 & 118 & 112 & Avg. \\ 
\midrule
\multirow{3}{*}{1/8x} & NeUS & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\
 & NeUS-BL & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\
 & BANF & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\ 
\midrule
\multirow{3}{*}{1/4x} & NeUS & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\
 & NeUS-BL & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\
 & BANF & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\ 
\midrule
\multirow{3}{*}{1/2x} & NeUS & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\
 & NeUS-BL & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\
 & BANF & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\ 
\midrule
\multirow{3}{*}{1x} & NeUS & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\
 & NeUS-BL & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\
 & BANF & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\ 
\midrule
\multirow{3}{*}{Avg.} & NeUS & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\
 & NeUS-BL & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\
 & BANF & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- & -/- \\
\bottomrule
\end{tabular}
\caption{3D Surface Results on the DTU Dataset. We denote band-limited NeUS as NeUS-BL and compare across multiple scales.}
\label{tab:3d}
\end{table*}



==> tab/abl1.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{cc}
% \toprule
Experiment & Chamfer ($\times 10^2) $~$\downarrow$ \\ \midrule
w/o Color MLP Feat. Input & 11.9 \\
w/o  Resolution Warmup & 13.6 \\
BANF & \textbf{11.4}
% \\ \bottomrule
\end{tabular}
% \caption{Color MLP Input and Resolution Warmup Ablations for Inverse Rendering.}
\label{tab:abl1}
\end{table}

==> tab/abl2.tex <==
\begin{table}[]
\centering
\begin{tabular}{cc}
Color MLP Training & Chamfer \\ \midrule
Cascaded & 9.16 \\
Direct & \textbf{8.19}
\end{tabular}
\caption{Color MLP Training Ablation for Inverse Rendering. We evaluate on the Blender dataset~\cite{barron2021mipnerf} averaged over all objects, evaluated at 1/4x.}
\label{tab:abl2}
\end{table}
